Adaptive Multi-Corpora Language Model Training for Speech Recognition

Neural network language model (NNLM) plays an essential role in automatic speech recognition (ASR) systems, especially in adaptation tasks when text-only data is available. In practice, an NNLM is typically trained on a combination of data sampled from multiple corpora. Thus, the data sampling strategy is important to the adaptation performance. Most existing works focus on designing static sampling strategies. However, each corpus may show varying impacts at different NNLM training stages. In this paper, we introduce a novel adaptive multi-corpora training algorithm that dynamically learns and adjusts the sampling probability of each corpus along the training process. The algorithm is robust to corpora sizes and domain relevance. Compared with static sampling strategy baselines, the proposed approach yields remarkable improvement by achieving up to relative 7% and 9% word error rate (WER) reductions on in-domain and out-of-domain adaptation tasks, respectively.

==> Definitions.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{url}
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm2e}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

%\newcommand{\ab}{\mathbf{a}}
%\newcommand{\bb}{\mathbf{b}}
%\newcommand{\cbb}{\mathbf{c}}
%\newcommand{\db}{\mathbf{d}}
%\newcommand{\eb}{\mathbf{e}}
%\newcommand{\fb}{\mathbf{f}}
%\newcommand{\gb}{\mathbf{g}}
%\newcommand{\hb}{\mathbf{h}}
%\newcommand{\ib}{\mathbf{i}}
%\newcommand{\jb}{\mathbf{j}}
%\newcommand{\kb}{\mathbf{k}}
%\newcommand{\lb}{\mathbf{l}}
%\newcommand{\mb}{\mathbf{m}}
%\newcommand{\nbb}{\mathbf{n}}
%\newcommand{\ob}{\mathbf{o}}
%\newcommand{\pb}{\mathbf{p}}
%\newcommand{\qb}{\mathbf{q}}
%\newcommand{\rb}{\mathbf{r}}
%\newcommand{\sbb}{\mathbf{s}}
%\newcommand{\tb}{\mathbf{t}}
%\newcommand{\ub}{\mathbf{u}}
%\newcommand{\vb}{\mathbf{v}}
%\newcommand{\wb}{\mathbf{w}}
%\newcommand{\xb}{\mathbf{x}}
%\newcommand{\yb}{\mathbf{y}}
%\newcommand{\zb}{\mathbf{z}}
%
%\newcommand{\abtil}{\tilde{\ab}}
%\newcommand{\bbtil}{\tilde{\bb}}
%\newcommand{\cbtil}{\tilde{\cbb}}
%\newcommand{\dbtil}{\tilde{\db}}
%\newcommand{\ebtil}{\tilde{\eb}}
%\newcommand{\fbtil}{\tilde{\fb}}
%\newcommand{\gbtil}{\tilde{\gb}}
%\newcommand{\hbtil}{\tilde{\hb}}
%\newcommand{\ibtil}{\tilde{\ib}}
%\newcommand{\jbtil}{\tilde{\jb}}
%\newcommand{\kbtil}{\tilde{\kb}}
%\newcommand{\lbtil}{\tilde{\lb}}
%\newcommand{\mbtil}{\tilde{\mb}}
%\newcommand{\nbtil}{\tilde{\nbb}}
%\newcommand{\obtil}{\tilde{\ob}}
%\newcommand{\pbtil}{\tilde{\pb}}
%\newcommand{\qbtil}{\tilde{\qb}}
%\newcommand{\rbtil}{\tilde{\rb}}
%\newcommand{\sbtil}{\tilde{\sbb}}
%\newcommand{\tbtil}{\tilde{\tb}}
%\newcommand{\ubtil}{\tilde{\ub}}
%\newcommand{\vbtil}{\tilde{\vb}}
%\newcommand{\wbtil}{\tilde{\wb}}
%\newcommand{\xbtil}{\tilde{\xb}}
%\newcommand{\ybtil}{\tilde{\yb}}
%\newcommand{\zbtil}{\tilde{\zb}}
%
%
%\newcommand{\atil}{\tilde{a}}
%\newcommand{\btil}{\tilde{b}}
%\newcommand{\ctil}{\tilde{c}}
%\newcommand{\dtil}{\tilde{d}}
%\newcommand{\etil}{\tilde{e}}
%\newcommand{\ftil}{\tilde{f}}
%\newcommand{\gtil}{\tilde{g}}
%\newcommand{\htil}{\tilde{h}}
%\newcommand{\itil}{\tilde{i}}
%\newcommand{\jtil}{\tilde{j}}
%\newcommand{\ktil}{\tilde{k}}
%\newcommand{\ltil}{\tilde{l}}
%\newcommand{\mtil}{\tilde{m}}
%\newcommand{\ntil}{\tilde{n}}
%\newcommand{\otil}{\tilde{o}}
%\newcommand{\ptil}{\tilde{p}}
%\newcommand{\qtil}{\tilde{q}}
%\newcommand{\rtil}{\tilde{r}}
%\newcommand{\stil}{\tilde{s}}
%\newcommand{\ttil}{\tilde{t}}
%\newcommand{\util}{\tilde{u}}
%\newcommand{\vtil}{\tilde{v}}
%\newcommand{\wtil}{\tilde{w}}
%\newcommand{\xtil}{\tilde{x}}
%\newcommand{\ytil}{\tilde{y}}
%\newcommand{\ztil}{\tilde{z}}
%
%\newcommand{\Atil}{\tilde{A}}
%\newcommand{\Btil}{\tilde{B}}
%\newcommand{\Ctil}{\tilde{C}}
%\newcommand{\Dtil}{\tilde{D}}
%\newcommand{\Etil}{\tilde{E}}
%\newcommand{\Ftil}{\tilde{F}}
%\newcommand{\Gtil}{\tilde{G}}
%\newcommand{\Htil}{\tilde{H}}
%\newcommand{\Itil}{\tilde{I}}
%\newcommand{\Jtil}{\tilde{J}}
%\newcommand{\Ktil}{\tilde{K}}
%\newcommand{\Ltil}{\tilde{L}}
%\newcommand{\Mtil}{\tilde{M}}
%\newcommand{\Ntil}{\tilde{N}}
%\newcommand{\Otil}{\tilde{O}}
%\newcommand{\Ptil}{\tilde{P}}
%\newcommand{\Qtil}{\tilde{Q}}
%\newcommand{\Rtil}{\tilde{R}}
%\newcommand{\Stil}{\tilde{S}}
%\newcommand{\Ttil}{\tilde{T}}
%\newcommand{\Util}{\tilde{U}}
%\newcommand{\Vtil}{\tilde{V}}
%\newcommand{\Wtil}{\tilde{W}}
%\newcommand{\Xtil}{\tilde{X}}
%\newcommand{\Ytil}{\tilde{Y}}
%\newcommand{\Ztil}{\tilde{Z}}
%
%\newcommand{\abar}{\bar{a}}
%\newcommand{\bbar}{\bar{b}}
%\newcommand{\cbar}{\bar{c}}
%\newcommand{\dbar}{\bar{d}}
%\newcommand{\ebar}{\bar{e}}
%\newcommand{\fbar}{\bar{f}}
%\newcommand{\gbar}{\bar{g}}
%\newcommand{\hbr}{\bar{h}}
%\newcommand{\ibar}{\bar{i}}
%\newcommand{\jbar}{\bar{j}}
%\newcommand{\kbar}{\bar{k}}
%\newcommand{\lbar}{\bar{l}}
%\newcommand{\mbar}{\bar{m}}
%\newcommand{\nbar}{\bar{n}}
%\newcommand{\obar}{\bar{o}}
%\newcommand{\pbar}{\bar{p}}
%\newcommand{\qbar}{\bar{q}}
%\newcommand{\rbar}{\bar{r}}
%\newcommand{\sbar}{\bar{s}}
%\newcommand{\tbar}{\bar{t}}
%\newcommand{\ubar}{\bar{u}}
%\newcommand{\vbar}{\bar{v}}
%\newcommand{\wbar}{\bar{w}}
%\newcommand{\xbar}{\bar{x}}
%\newcommand{\ybar}{\bar{y}}
%\newcommand{\zbar}{\bar{z}}
%
%\newcommand{\abbar}{\bar{\ab}}
%\newcommand{\bbbar}{\bar{\bb}}
%\newcommand{\cbbar}{\bar{\cb}}
%\newcommand{\dbbar}{\bar{\db}}
%\newcommand{\ebbar}{\bar{\eb}}
%\newcommand{\fbbar}{\bar{\fb}}
%\newcommand{\gbbar}{\bar{\gb}}
%\newcommand{\hbbar}{\bar{\hb}}
%\newcommand{\ibbar}{\bar{\ib}}
%\newcommand{\jbbar}{\bar{\jb}}
%\newcommand{\kbbar}{\bar{\kb}}
%\newcommand{\lbbar}{\bar{\lb}}
%\newcommand{\mbbar}{\bar{\mb}}
%\newcommand{\nbbar}{\bar{\nbb}}
%\newcommand{\obbar}{\bar{\ob}}
%\newcommand{\pbbar}{\bar{\pb}}
%\newcommand{\qbbar}{\bar{\qb}}
%\newcommand{\rbbar}{\bar{\rb}}
%\newcommand{\sbbar}{\bar{\sbb}}
%\newcommand{\tbbar}{\bar{\tb}}
%\newcommand{\ubbar}{\bar{\ub}}
%\newcommand{\vbbar}{\bar{\vb}}
%\newcommand{\wbbar}{\bar{\wb}}
%\newcommand{\xbbar}{\bar{\xb}}
%\newcommand{\ybbar}{\bar{\yb}}
%\newcommand{\zbbar}{\bar{\zb}}
%
%\newcommand{\Ab}{\mathbf{A}}
%\newcommand{\Bb}{\mathbf{B}}
%\newcommand{\Cb}{\mathbf{C}}
%\newcommand{\Db}{\mathbf{D}}
%\newcommand{\Eb}{\mathbf{E}}
%\newcommand{\Fb}{\mathbf{F}}
%\newcommand{\Gb}{\mathbf{G}}
%\newcommand{\Hb}{\mathbf{H}}
%\newcommand{\Ib}{\mathbf{I}}
%\newcommand{\Jb}{\mathbf{J}}
%\newcommand{\Kb}{\mathbf{K}}
%\newcommand{\Lb}{\mathbf{L}}
%\newcommand{\Mb}{\mathbf{M}}
%\newcommand{\Nb}{\mathbf{N}}
%\newcommand{\Ob}{\mathbf{O}}
%\newcommand{\Pb}{\mathbf{P}}
%\newcommand{\Qb}{\mathbf{Q}}
%\newcommand{\Rb}{\mathbf{R}}
%\newcommand{\Sbb}{\mathbf{S}}
%\newcommand{\Tb}{\mathbf{T}}
%\newcommand{\Ub}{\mathbf{U}}
%\newcommand{\Vb}{\mathbf{V}}
%\newcommand{\Wb}{\mathbf{W}}
%\newcommand{\Xb}{\mathbf{X}}
%\newcommand{\Yb}{\mathbf{Y}}
%\newcommand{\Zb}{\mathbf{Z}}
%
%\newcommand{\Abtil}{\tilde{\Ab}}
%\newcommand{\Bbtil}{\tilde{\Bb}}
%\newcommand{\Cbtil}{\tilde{\Cb}}
%\newcommand{\Dbtil}{\tilde{\Db}}
%\newcommand{\Ebtil}{\tilde{\Eb}}
%\newcommand{\Fbtil}{\tilde{\Fb}}
%\newcommand{\Gbtil}{\tilde{\Gb}}
%\newcommand{\Hbtil}{\tilde{\Hb}}
%\newcommand{\Ibtil}{\tilde{\Ib}}
%\newcommand{\Jbtil}{\tilde{\Jb}}
%\newcommand{\Kbtil}{\tilde{\Kb}}
%\newcommand{\Lbtil}{\tilde{\Lb}}
%\newcommand{\Mbtil}{\tilde{\Mb}}
%\newcommand{\Nbtil}{\tilde{\Nb}}
%\newcommand{\Obtil}{\tilde{\Ob}}
%\newcommand{\Pbtil}{\tilde{\Pb}}
%\newcommand{\Qbtil}{\tilde{\Qb}}
%\newcommand{\Rbtil}{\tilde{\Rb}}
%\newcommand{\Sbtil}{\tilde{\Sbb}}
%\newcommand{\Tbtil}{\tilde{\Tb}}
%\newcommand{\Ubtil}{\tilde{\Ub}}
%\newcommand{\Vbtil}{\tilde{\Vb}}
%\newcommand{\Wbtil}{\tilde{\Wb}}
%\newcommand{\Xbtil}{\tilde{\Xb}}
%\newcommand{\Ybtil}{\tilde{\Yb}}
%\newcommand{\Zbtil}{\tilde{\Zb}}
%
%\newcommand{\Abar}{\bar{A}}
%\newcommand{\Bbar}{\bar{B}}
%\newcommand{\Cbar}{\bar{C}}
%\newcommand{\Dbar}{\bar{D}}
%\newcommand{\Ebar}{\bar{E}}
%\newcommand{\Fbar}{\bar{F}}
%\newcommand{\Gbar}{\bar{G}}
%\newcommand{\Hbar}{\bar{H}}
%\newcommand{\Ibar}{\bar{I}}
%\newcommand{\Jbar}{\bar{J}}
%\newcommand{\Kbar}{\bar{K}}
%\newcommand{\Lbar}{\bar{L}}
%\newcommand{\Mbar}{\bar{M}}
%\newcommand{\Nbar}{\bar{N}}
%\newcommand{\Obar}{\bar{O}}
%\newcommand{\Pbar}{\bar{P}}
%\newcommand{\Qbar}{\bar{Q}}
%\newcommand{\Rbar}{\bar{R}}
%\newcommand{\Sbar}{\bar{S}}
%\newcommand{\Tbar}{\bar{T}}
%\newcommand{\Ubar}{\bar{U}}
%\newcommand{\Vbar}{\bar{V}}
%\newcommand{\Wbar}{\bar{W}}
%\newcommand{\Xbar}{\bar{X}}
%\newcommand{\Ybar}{\bar{Y}}
%\newcommand{\Zbar}{\bar{Z}}
%
%\newcommand{\Abbar}{\bar{\Ab}}
%\newcommand{\Bbbar}{\bar{\Bb}}
%\newcommand{\Cbbar}{\bar{\Cb}}
%\newcommand{\Dbbar}{\bar{\Db}}
%\newcommand{\Ebbar}{\bar{\Eb}}
%\newcommand{\Fbbar}{\bar{\Fb}}
%\newcommand{\Gbbar}{\bar{\Gb}}
%\newcommand{\Hbbar}{\bar{\Hb}}
%\newcommand{\Ibbar}{\bar{\Ib}}
%\newcommand{\Jbbar}{\bar{\Jb}}
%\newcommand{\Kbbar}{\bar{\Kb}}
%\newcommand{\Lbbar}{\bar{\Lb}}
%\newcommand{\Mbbar}{\bar{\Mb}}
%\newcommand{\Nbbar}{\bar{\Nb}}
%\newcommand{\Obbar}{\bar{\Ob}}
%\newcommand{\Pbbar}{\bar{\Pb}}
%\newcommand{\Qbbar}{\bar{\Qb}}
%\newcommand{\Rbbar}{\bar{\Rb}}
%\newcommand{\Sbbar}{\bar{\Sb}}
%\newcommand{\Tbbar}{\bar{\Tb}}
%\newcommand{\Ubbar}{\bar{\Ub}}
%\newcommand{\Vbbar}{\bar{\Vb}}
%\newcommand{\Wbbar}{\bar{\Wb}}
%\newcommand{\Xbbar}{\bar{\Xb}}
%\newcommand{\Ybbar}{\bar{\Yb}}
%\newcommand{\Zbbar}{\bar{\Zb}}
%
%\newcommand{\Ahat}{\hat{A}}
%\newcommand{\Bhat}{\hat{B}}
%\newcommand{\Chat}{\hat{C}}
%\newcommand{\Dhat}{\hat{D}}
%\newcommand{\Ehat}{\hat{E}}
%\newcommand{\Fhat}{\hat{F}}
%\newcommand{\Ghat}{\hat{G}}
%\newcommand{\Hhat}{\hat{H}}
%\newcommand{\Ihat}{\hat{I}}
%\newcommand{\Jhat}{\hat{J}}
%\newcommand{\Khat}{\hat{K}}
%\newcommand{\Lhat}{\hat{L}}
%\newcommand{\Mhat}{\hat{M}}
%\newcommand{\Nhat}{\hat{N}}
%\newcommand{\Ohat}{\hat{O}}
%\newcommand{\Phat}{\hat{P}}
%\newcommand{\Qhat}{\hat{Q}}
%\newcommand{\Rhat}{\hat{R}}
%\newcommand{\Shat}{\hat{S}}
%\newcommand{\That}{\hat{T}}
%\newcommand{\Uhat}{\hat{U}}
%\newcommand{\Vhat}{\hat{V}}
%\newcommand{\What}{\hat{W}}
%\newcommand{\Xhat}{\hat{X}}
%\newcommand{\Yhat}{\hat{Y}}
%\newcommand{\Zhat}{\hat{Z}}
%
%\newcommand{\Abhat}{\hat{\Ab}}
%\newcommand{\Bbhat}{\hat{\Bb}}
%\newcommand{\Cbhat}{\hat{\Cb}}
%\newcommand{\Dbhat}{\hat{\Db}}
%\newcommand{\Ebhat}{\hat{\Eb}}
%\newcommand{\Fbhat}{\hat{\Fb}}
%\newcommand{\Gbhat}{\hat{\Gb}}
%\newcommand{\Hbhat}{\hat{\Hb}}
%\newcommand{\Ibhat}{\hat{\Ib}}
%\newcommand{\Jbhat}{\hat{\Jb}}
%\newcommand{\Kbhat}{\hat{\Kb}}
%\newcommand{\Lbhat}{\hat{\Lb}}
%\newcommand{\Mbhat}{\hat{\Mb}}
%\newcommand{\Nbhat}{\hat{\Nb}}
%\newcommand{\Obhat}{\hat{\Ob}}
%\newcommand{\Pbhat}{\hat{\Pb}}
%\newcommand{\Qbhat}{\hat{\Qb}}
%\newcommand{\Rbhat}{\hat{\Rb}}
%\newcommand{\Sbhat}{\hat{\Sb}}
%\newcommand{\Tbhat}{\hat{\Tb}}
%\newcommand{\Ubhat}{\hat{\Ub}}
%\newcommand{\Vbhat}{\hat{\Vb}}
%\newcommand{\Wbhat}{\hat{\Wb}}
%\newcommand{\Xbhat}{\hat{\Xb}}
%\newcommand{\Ybhat}{\hat{\Yb}}
%\newcommand{\Zbhat}{\hat{\Zb}}
%
%\newcommand{\Acal}{\mathcal{A}}
%\newcommand{\Bcal}{\mathcal{B}}
%\newcommand{\Ccal}{\mathcal{C}}
%\newcommand{\Dcal}{\mathcal{D}}
%\newcommand{\Ecal}{\mathcal{E}}
%\newcommand{\Fcal}{\mathcal{F}}
%\newcommand{\Gcal}{\mathcal{G}}
%\newcommand{\Hcal}{\mathcal{H}}
%\newcommand{\Ical}{\mathcal{I}}
%\newcommand{\Jcal}{\mathcal{J}}
%\newcommand{\Kcal}{\mathcal{K}}
%\newcommand{\Lcal}{\mathcal{L}}
%\newcommand{\Mcal}{\mathcal{M}}
%\newcommand{\Ncal}{\mathcal{N}}
%\newcommand{\Ocal}{\mathcal{O}}
%\newcommand{\Pcal}{\mathcal{P}}
%\newcommand{\Qcal}{\mathcal{Q}}
%\newcommand{\Rcal}{\mathcal{R}}
%\newcommand{\Scal}{{\mathcal{S}}}
%\newcommand{\Tcal}{{\mathcal{T}}}
%\newcommand{\Ucal}{\mathcal{U}}
%\newcommand{\Vcal}{\mathcal{V}}
%\newcommand{\Wcal}{\mathcal{W}}
%\newcommand{\Xcal}{\mathcal{X}}
%\newcommand{\Ycal}{\mathcal{Y}}
%\newcommand{\Zcal}{\mathcal{Z}}
%
%\newcommand{\Atilde}{\widetilde{A}}
%\newcommand{\Btilde}{\widetilde{B}}
%\newcommand{\Ctilde}{\widetilde{C}}
%\newcommand{\Dtilde}{\widetilde{D}}
%\newcommand{\Etilde}{\widetilde{E}}
%\newcommand{\Ftilde}{\widetilde{F}}
%\newcommand{\Gtilde}{\widetilde{G}}
%\newcommand{\Htilde}{\widetilde{H}}
%\newcommand{\Itilde}{\widetilde{I}}
%\newcommand{\Jtilde}{\widetilde{J}}
%\newcommand{\Ktilde}{\widetilde{K}}
%\newcommand{\Ltilde}{\widetilde{L}}
%\newcommand{\Mtilde}{\widetilde{M}}
%\newcommand{\Ntilde}{\widetilde{N}}
%\newcommand{\Otilde}{\widetilde{O}}
%\newcommand{\Ptilde}{\widetilde{P}}
%\newcommand{\Qtilde}{\widetilde{Q}}
%\newcommand{\Rtilde}{\widetilde{R}}
%\newcommand{\Stilde}{\widetilde{S}}
%\newcommand{\Ttilde}{\widetilde{T}}
%\newcommand{\Utilde}{\widetilde{U}}
%\newcommand{\Vtilde}{\widetilde{V}}
%\newcommand{\Wtilde}{\widetilde{W}}
%\newcommand{\Xtilde}{\widetilde{X}}
%\newcommand{\Ytilde}{\widetilde{Y}}
%\newcommand{\Ztilde}{\widetilde{Z}}
%
%
%%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%
%
%\newcommand{\CC}{\mathbb{C}} % Complex numbers
%\newcommand{\EE}{\mathbb{E}} % Expectation
%\newcommand{\II}{\mathbb{I}} % Delta Indicator
%\newcommand{\VV}{\mathbb{V}} % Variance
%\newcommand{\KK}{\mathbb{K}} % Arbitrary field
%\newcommand{\MM}{\mathbb{M}} % Median
%\newcommand{\NN}{\mathbb{N}} % Natural numbers
%\newcommand{\PP}{\mathbb{P}} % Probability
%\newcommand{\QQ}{\mathbb{Q}} % Rationals
%\newcommand{\RR}{\mathbb{R}} % Real numbers
%\newcommand{\ZZ}{\mathbb{Z}} % Integers
%\newcommand{\XX}{\mathbb{X}} % Integers
%\newcommand{\YY}{\mathbb{Y}} % Integers
%
%\newcommand{\one}{\mathbf{1}}  % Identity
%\newcommand{\zero}{\mathbf{0}} % Zero
%%\newcommand{\TRUE}{\mathbf{TRUE}}  % True
%%\newcommand{\FALSE}{\mathbf{FALSE}}  % False
%
%\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
%\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
%\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
%\newcommand{\sgn}{\mathop{\mathrm{sign}}}
%\newcommand{\tr}{\mathop{\mathrm{tr}}}
%\newcommand{\diag}{\mathop{\mathrm{diag}}}
%\newcommand{\rank}{\mathop{\mathrm{rank}}}
%%\newcommand{\ovec}{\mathop{\mathrm{vec}}}
%\newcommand{\traj}{\mathop{\mathrm{Traj}}}
%\newcommand*{\cov}{\mathrm{Cov}}
%\newcommand*{\conv}{\mathrm{conv}}
%\newcommand*{\const}{\mathrm{constant}}
%
%%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
%\newcommand{\sigmab}{\bm{\sigma}}
%\newcommand{\Sigmab}{\mathbf{\Sigma}}
%
%
%%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%
%
%%% Some style files might actually define these variables.
%%% So don't mess with them if they are already defined
%
%\ifx\BlackBox\undefined
%\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
%\fi
%
%\ifx\QED\undefined
%\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
%\fi
%
%\ifx\proof\undefined
%\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%%\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
%\fi
%
%\ifx\theorem\undefined
%\newtheorem{theorem}{Theorem}
%\newtheorem{example}{Example}
%\newtheorem{property}{Property}
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{conjecture}[theorem]{Conjecture}
%\fi
%
%\ifx\axiom\undefined
%\newtheorem{axiom}[theorem]{Axiom}
%\fi
%
%%%%%%%%% Utility functions %%%%%%%%%%%%%%%
%
%\newcommand{\eq}[1]{(\ref{#1})}
%\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
%\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
%\newcommand{\mydet}[1]{\det\left[ #1 \right]}
%\newcommand{\sembrack}[1]{[\![#1]\!]}
%
%\newcommand{\ea}{\emph{et al.}}
%\newcommand{\eg}{\emph{e.g.}}
%\newcommand{\ie}{\emph{i.e.}}
%\newcommand{\iid}{\emph{iid}}
%
%%\newcommand{\alex}[1]{{\bf ALEX: \uppercase{#1}}}
%%\newcommand{\vishy}[1]{{\bf VISHY: \uppercase{#1}}}
%%\newcommand{\rene}[1]{{\bf RENE: \uppercase{#1}}}
%%\newcommand{\karsten}[1]{{\bf KARSTEN: \uppercase{#1}}}
%
%%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%
%
%\newcommand{\methodname}{KDE}
%\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
%
%\newcommand{\hsic}{\mathrm{HSIC}}
%\newcommand{\mmd}{\mathrm{MMD}}
%
%%\newcommand{\tDiag}{\textsf{Diag}}
%%\newcommand{\tTr}{\textsf{Tr}}
%%\newcommand{\tE}{\textsf{E}}
%%\newcommand{\tVec}{\textsf{Vec}}
%%\newcommand{\tRank}{\textsf{Rank}}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% math symbols and commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\newcommand{\eq}[1]{(\ref{#1})}
%%\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
%
%%brackets
%\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
%\newcommand{\rbr}[1]{\left(#1\right)}
%\newcommand{\sbr}[1]{\left[#1\right]}
%\newcommand{\cbr}[1]{\left\{#1\right\}}
%\newcommand{\nbr}[1]{\left\|#1\right\|}
%\newcommand{\abr}[1]{\left|#1\right|}
%\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
%\renewcommand{\url}[1]{{\sffamily #1}}
%\newcommand{\arow}[2]{#1_{#2\cdot}}
%\newcommand{\acol}[2]{#1_{\cdot#2}}
%
%\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
%\def\ci{\perp\!\!\!\perp}
%
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "./SIGMOD06/SIGMODB06.tex"
%%%% End:
%
%
%% by xinhua
%\newcommand{\delhat}{\hat{\delta}}
%\newcommand{\delbar}{\bar{\delta}}
%\newcommand{\HH}{\mathbb{H}} % Arbitrary field
%\newcommand{\ve}{\varepsilon}
%\newcommand{\dom}{\mathrm{dom}}
%
%%%% Local Variables:
%%%% mode: latex
%%%% TeX-master: "./SIGMOD06/SIGMODB06.tex"
%%%% End:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%                               PROOF, THEOREM, and FRIENDS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
%%\newenvironment{proof}{\par\noindent{\bf Proof.\ }}{\hfill\BlackBox\\[2mm]}
%
%%\newcounter{all_counter}
%%\newcounter{lemma_counter}
%%\newcounter{proposition_counter}
%%\newcounter{remark_counter}
%%\newcounter{corollary_counter}
%%\newcounter{definition_counter}
%%\newcounter{conjecture_counter}
%%\newcounter{axiom_counter}
%%
%%\setcounter{lemma_counter}{0} \setcounter{proposition_counter}{0}
%%\setcounter{remark_counter}{0} \setcounter{corollary_counter}{0}
%%\setcounter{definition_counter}{0}
%%\setcounter{conjecture_counter}{0} \setcounter{axiom_counter}{0}
%
%%\newtheorem{lemma}[lemma_counter]{Lemma}
%%\newtheorem{proposition}[proposition_counter]{Proposition}
%%\newtheorem{remark}[remark_counter]{Remark}
%%\newtheorem{corollary}[corollary_counter]{Corollary}
%%\newtheorem{definition}[definition_counter]{Definition}
%%\newtheorem{conjecture}[conjecture_counter]{Conjecture}
%%\newtheorem{axiom}[axiom_counter]{Axiom}
%
%\newtheorem{assumption}[theorem]{Assumption}
%
%\newcommand{\ahat}{\hat{a}}
%\newcommand{\bhat}{\hat{b}}
%\newcommand{\chat}{\hat{c}}
%\newcommand{\dhat}{\hat{d}}
%\newcommand{\ehat}{\hat{e}}
%\newcommand{\fhat}{\hat{f}}
%\newcommand{\ghat}{\hat{g}}
%\newcommand{\hhat}{\hat{h}}
%\newcommand{\ihat}{\hat{i}}
%\newcommand{\jhat}{\hat{j}}
%\newcommand{\khat}{\hat{k}}
%\newcommand{\lhat}{\hat{l}}
%\newcommand{\mhat}{\hat{m}}
%\newcommand{\nhat}{\hat{n}}
%\newcommand{\ohat}{\hat{o}}
%\newcommand{\phat}{\hat{p}}
%\newcommand{\qhat}{\hat{q}}
%\newcommand{\rhat}{\hat{r}}
%\newcommand{\shat}{\hat{s}}
%\newcommand{\that}{\hat{t}}
%\newcommand{\uhat}{\hat{u}}
%\newcommand{\vhat}{\hat{v}}
%\newcommand{\what}{\hat{w}}
%\newcommand{\xhat}{\hat{x}}
%\newcommand{\yhat}{\hat{y}}
%\newcommand{\zhat}{\hat{z}}
%
%\newcommand{\abhat}{\hat{\ab}}
%\newcommand{\bbhat}{\hat{\bb}}
%\newcommand{\cbhat}{\hat{\cb}}
%\newcommand{\dbhat}{\hat{\db}}
%\newcommand{\ebhat}{\hat{\eb}}
%\newcommand{\fbhat}{\hat{\fb}}
%\newcommand{\gbhat}{\hat{\gb}}
%\newcommand{\hbhat}{\hat{\hb}}
%\newcommand{\ibhat}{\hat{\ib}}
%\newcommand{\jbhat}{\hat{\jb}}
%\newcommand{\kbhat}{\hat{\kb}}
%\newcommand{\lbhat}{\hat{\lb}}
%\newcommand{\mbhat}{\hat{\mb}}
%\newcommand{\nbhat}{\hat{\nb}}
%\newcommand{\obhat}{\hat{\ob}}
%\newcommand{\pbhat}{\hat{\pb}}
%\newcommand{\qbhat}{\hat{\qb}}
%\newcommand{\rbhat}{\hat{\rb}}
%\newcommand{\sbhat}{\hat{\sb}}
%\newcommand{\tbhat}{\hat{\tb}}
%\newcommand{\ubhat}{\hat{\ub}}
%\newcommand{\vbhat}{\hat{\vb}}
%\newcommand{\wbhat}{\hat{\wb}}
%\newcommand{\xbhat}{\hat{\xb}}
%\newcommand{\ybhat}{\hat{\yb}}
%\newcommand{\zbhat}{\hat{\zb}}
%
%\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}
%
%\newcommand{\avec}{\vec{a}}
%\newcommand{\bvec}{\vec{b}}
%\newcommand{\cvec}{\vec{c}}
%\newcommand{\dvec}{\vec{d}}
%\newcommand{\evec}{\vec{e}}
%\newcommand{\fvec}{\vec{f}}
%\newcommand{\gvec}{\vec{g}}
%\newcommand{\hvec}{\vec{h}}
%\newcommand{\ivec}{\vec{i}}
%\newcommand{\jvec}{\vec{j}}
%\newcommand{\kvec}{\vec{k}}
%\newcommand{\lvec}{\vec{l}}
%\newcommand{\mvec}{\vec{m}}
%\newcommand{\nvec}{\vec{n}}
%\newcommand{\ovec}{\vec{o}}
%\newcommand{\pvec}{\vec{p}}
%\newcommand{\qvec}{\vec{q}}
%\newcommand{\rvec}{\vec{r}}
%\newcommand{\svec}{\vec{s}}
%\newcommand{\tvec}{\vec{t}}
%\newcommand{\uvec}{\vec{u}}
%\newcommand{\vvec}{\vec{v}}
%\newcommand{\wvec}{\vec{w}}
%\newcommand{\xvec}{\vec{x}}
%\newcommand{\yvec}{\vec{y}}
%\newcommand{\zvec}{\vec{z}}
%
%\newcommand{\Avec}{\vec{A}}
%\newcommand{\Bvec}{\vec{B}}
%\newcommand{\Cvec}{\vec{C}}
%\newcommand{\Dvec}{\vec{D}}
%\newcommand{\Evec}{\vec{E}}
%\newcommand{\Fvec}{\vec{F}}
%\newcommand{\Gvec}{\vec{G}}
%\newcommand{\Hvec}{\vec{H}}
%\newcommand{\Ivec}{\vec{I}}
%\newcommand{\Jvec}{\vec{J}}
%\newcommand{\Kvec}{\vec{K}}
%\newcommand{\Lvec}{\vec{L}}
%\newcommand{\Mvec}{\vec{M}}
%\newcommand{\Nvec}{\vec{N}}
%\newcommand{\Ovec}{\vec{O}}
%\newcommand{\Pvec}{\vec{P}}
%\newcommand{\Qvec}{\vec{Q}}
%\newcommand{\Rvec}{\vec{R}}
%\newcommand{\Svec}{\vec{S}}
%\newcommand{\Tvec}{\vec{T}}
%\newcommand{\Uvec}{\vec{U}}
%\newcommand{\Vvec}{\vec{V}}
%\newcommand{\Wvec}{\vec{W}}
%\newcommand{\Xvec}{\vec{X}}
%\newcommand{\Yvec}{\vec{Y}}
%\newcommand{\Zvec}{\vec{Z}}
%
%
%\newcommand{\alphavec}{\vec{\alpha}}
%\newcommand{\betavec}{\vec{\beta}}
%\newcommand{\deltavec}{\vec{\delta}}
%\newcommand{\etavec}{\vec{\eta}}
%\newcommand{\phivec}{\vec{\phi}}
%\newcommand{\psivec}{\vec{\psi}}
%\newcommand{\thetavec}{\vec{\theta}}
%\newcommand{\muvec}{\vec{\mu}}
%\newcommand{\xivec}{\vec{\xi}}
%
%
%\newcommand{\alphab}{\boldsymbol{\alpha}}
%\newcommand{\betab}{\boldsymbol{\beta}}
%\newcommand{\gammab}{\boldsymbol{\gamma}}
%\newcommand{\thetab}{\boldsymbol{\theta}}
%\newcommand{\mub}{\boldsymbol{\mu}}
%\newcommand{\xib}{\boldsymbol{\xi}}
%\newcommand{\Deltab}{\boldsymbol{\Delta}}
%\newcommand{\Pib}{\boldsymbol{\Pi}}
%\newcommand{\etab}{\boldsymbol{\eta}}
%\newcommand{\taub}{\boldsymbol{\tau}}
%\newcommand{\lambdab}{\boldsymbol{\lambda}}
%\newcommand{\pitil}{\tilde{\pi}}
%
%\newcommand{\rmd}{\mathrm{d}}
%\newcommand{\HSIC}{\mathrm{HSIC}}
%
%\newcommand{\dir}{\mathrm{Dir}}
%\newcommand{\dirp}{\mathrm{DP}}
%\newcommand{\multi}{\mathrm{Multi}}
%\newcommand{\gam}{\mathrm{Gamma}}
%\newcommand{\var}{\mathrm{Var}}
%\newcommand{\cor}{\mathrm{Corr}}
%\newcommand{\bet}{\mathrm{Beta}}
%
%\newcommand{\ra}{\rightarrow}
%
%\newcommand{\idf}{{\tt idf}}
%
%\newcommand{\tp}{\text{tp}}
%\newcommand{\fn}{\text{fn}}
%\newcommand{\fp}{\text{fp}}
%\newcommand{\tpb}{\overline{\text{tp}}}
%\newcommand{\fnb}{\overline{\text{fn}}}
%\newcommand{\fpb}{\overline{\text{fp}}}
%\newcommand{\pre}{\text{Pre}}
%\newcommand{\rec}{\text{Rec}}
%\newcommand{\fs}{\text{F-score}}
%\newcommand{\opt}{\text{opt}}
%
%\newcommand{\topics}{{\tt topics}}
%\newcommand{\industries}{{\tt industries}}
%\newcommand{\regions}{{\tt regions}}
%\newcommand{\ip}{{\tt ip}}
%\newcommand{\category}{{\tt category}}
%
%\newcommand{\grad}{{\nabla}}
%\newcommand{\gradbar}{{\bar{\nabla}}}
%\newcommand{\mbarr}{{\overline{M(r)}}}
%\newcommand{\card}{{\mathrm{card }}}
%\newcommand{\MED}{{\text{MED}}}
%\newcommand{\mubar}{\bar{\mu}}
%\newcommand{\emp}{{\mathrm{emp}}}
%\newcommand{\core}{{\mathrm{core}}}
%\newcommand{\zerob}{{\mathbf{0}}}
%\newcommand{\co}{{\mathrm{co}}}
%\newcommand{\argsup}{\mathop{\mathrm{argsup}}}
%\newcommand{\intr}{{\mathrm{int}}}
%\newcommand{\bd}{{\mathrm{bd}}}
%\newcommand{\BMRM}{{BMRM}}
%\newcommand{\where}{{\quad \text{where} \quad}}
%\newcommand{\lcg}{{\textit{l.c.g}}}
%\newcommand{\gradtil}{{\tilde{\grad}}}
%\newcommand{\alphabtil}{{\tilde{\alphab}}}
%\newcommand{\gstar}{{g^{\star}}}
%\newcommand{\fstar}{{f^{\star}}}
%
%
%\newcommand{\sqrttwo}{{\sqrt{2}}}
%\newcommand{\invsqrttwo}{{\frac{1}{\sqrt{2}}}}
%\newcommand{\invtwo}{{\frac{1}{2}}}
%\newcommand{\phihat}{{\hat{\phi}}}
%\newcommand{\cp}{\mathrm{cp}}
%\newcommand{\liblinear}{{\sf liblinear}}
%\newcommand{\lsbmrm}{{\sf ls-bmrm}}
%\newcommand{\qpbmrm}{{\sf qp-bmrm}}
%\newcommand{\pegasos}{{\sf pegasos}}
%\newcommand{\pegan}{{\sf pegasos-$n$}}
%\newcommand{\pegaone}{{\sf pegasos-1}}
%\newcommand{\nest}{{\sf Pragam}}
%\newcommand{\nestb}{{\sf Pragam-b}}
%\newcommand{\err}{{\sf err}}



\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}


\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\oobar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}




\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\alphavec}{\vec{\alpha}}
\newcommand{\alphavecbar}{\bar{\vec{\alpha}}}
\newcommand{\alphavechat}{\hat{\vec{\alpha}}}
\newcommand{\alphavectil}{\tilde{\vec{\alpha}}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}



\newcommand{\va}{{\tt a}}
\newcommand{\vc}{{\tt c}}
\newcommand{\vg}{{\tt g}}
\newcommand{\vp}{{\tt p}}
\newcommand{\vq}{{\tt q}}
\newcommand{\vs}{{\tt s}}
\newcommand{\vt}{{\tt t}}
\newcommand{\vu}{{\tt u}}
\newcommand{\vv}{{\tt v}}
\newcommand{\vw}{{\tt w}}
\newcommand{\vx}{{\tt x}}
\newcommand{\vy}{{\tt y}}
\newcommand{\val}{{\tt v}}


\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


%%%%%%%% Greek letters definitions %%%%%%%%%%%%%%%
\newcommand{\delhat}{\hat{\delta}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\ve}{\varepsilon}
\newcommand{\epsilonbar}{\bar{\epsilon}}
\newcommand{\etabar}{\bar{\eta}}
\newcommand{\Omegahat}{\hat{\Omega}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\Gammab}{\boldsymbol{\Gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\phib}{\boldsymbol{\phi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\rhob}{\boldsymbol{\rho}}
\newcommand{\sigmab}{\boldsymbol{\sigma}}
\newcommand{\Sigmab}{\boldsymbol{\Sigma}}

\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\pitil}{\tilde{\pi}}


%%%%%%%% Mathematical definitions %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\mathbb{R}}} % Real numbers
\newcommand{\ZZ}{\mathbb{Z}} % Integers
\newcommand{\XX}{\mathbb{X}} % Integers
\newcommand{\YY}{\mathbb{Y}} % Integers

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%
\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\vone}{\mathbf{1}}  % Identity
\newcommand{\vzero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\invtwo}{\frac{1}{2}}





%\newcommand{\TRUE}{\mathbf{TRUE}}  % True
%\newcommand{\FALSE}{\mathbf{FALSE}}  % False


%%%%%%%%%%%%%  Mathematical Operators  %%%%%%%%%%%%%%%

\DeclareMathOperator*{\mini}{\mathrm{minimize}}
\DeclareMathOperator*{\maxi}{\mathrm{maximize}}
\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\DeclareMathOperator*{\argmax}{\mathrm{argmax}}
\DeclareMathOperator*{\arginf}{\mathrm{arginf}}
\DeclareMathOperator*{\argsup}{\mathrm{argsup}}



%\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
%\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
%\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
%\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
%\newcommand{\sgn}{\mathop{\mathrm{sign}}}
%\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\trace}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
%\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\opvec}{\mathop{\mathrm{vec}}}
%\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand*{\cov}{\mathrm{Cov}}
\newcommand*{\covars}{\mathrm{Cov}}
\newcommand*{\conv}{\mathrm{conv}}
\newcommand*{\const}{\mathrm{constant}}
%\newcommand{\tDiag}{\textsf{Diag}}
%\newcommand{\tTr}{\textsf{Tr}}
%\newcommand{\tE}{\textsf{E}}
%\newcommand{\tVec}{\textsf{Vec}}
%\newcommand{\tRank}{\textsf{Rank}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}
\providecommand{\tra}{\intercal}
\newcommand{\ra}{\rightarrow}
\newcommand{\totvar}{\mathrm{TV}}


%%%%%%%% Thorems, Corollaries, etc %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
%\newenvironment{proof}{\emph{Proof. }}{ \hfill \QED}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{property}{Property}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{assumption}[theorem]{Assumption}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}
\newcommand{\mat}[1]{\mathbf{#1}}

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\etc}{\emph{etc.}}


%%%%%%%% Specific symbols for various projects %%%%%%%%%%%%%%%

\newcommand{\methodname}{KDE}
\newcommand{\hsic}{\mathrm{HSIC}}
\newcommand{\mmd}{\mathrm{MMD}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% math symbols and commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\eq}[1]{(\ref{#1})}
%\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\smallinner}[2]{{#1}^{\!\top}\!{#2}}  % no kernels allowed
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\nbrsub}[2]{\left\|#1\right\|_{#2}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\renewcommand{\url}[1]{{\sffamily #1}}
\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
%\newcommand{\grad}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

%%%%%%%%%%%%%%%%%%%%%%  Algorithmic  %%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\newcommand{\INPUT}{\STATE {\bfseries input}~}
\newcommand{\OUTPUT}{\STATE {\bfseries output}~}
\newcommand{\new}[1]{{\color{blue}\underline{\color{black}#1}}}
\newcommand{\comment}[1]{}


%%%%%%%%%%%%%%%%%%%%%%  Convex analysis related  %%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dom}{\mathrm{dom}\,}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\ri}{\mathrm{ri}\,}
\newcommand{\cl}{\mathrm{cl}\,}
\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}
\newcommand{\Fstar}{F^{\star}}
\newcommand{\Gstar}{G^{\star}}
\def\infconv{\phantom{.}_{\vee}\negthickspace\!\!^{+}}
\newcommand{\gr}{{\mathrm{gr}}}
\newcommand{\epi}{{\mathrm{epi}}}
\newcommand{\inte}{\mathrm{int}\,}
\newcommand{\aff}{\mathrm{aff}\,}
\newcommand{\cone}{\mathrm{cone}\,}


%%%%%%%%%%%%%%%%%%%%%%  Graphical model related  %%%%%%%%%%%%%%%%%%%%%%
\def\ci{\perp\!\!\!\perp}
\newcommand{\given}{\mathrm{|}}
\newcommand{\MRF}{\mathrm{MRF}}


%%%%%%%%%%%%%%%%%%%%%%  Distribution related  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Dir}{\mathrm{Dir}}
\newcommand{\dirp}{\mathrm{DP}}
\newcommand{\multi}{\mathrm{Multi}}
\newcommand{\gam}{\mathrm{Gamma}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cor}{\mathrm{Corr}}
\newcommand{\bet}{\mathrm{Beta}}
\newcommand{\convdist}{\,\mathop \rightarrow \limits^{\Dcal}\,}
\newcommand{\convprob}{\,\mathop \rightarrow \limits^{\mathbb{P}}\,}
\newcommand{\convlone}{\,\mathop \rightarrow \limits^{L_1}\,}
\newcommand{\convlp}{\,\mathop \rightarrow \limits^{L_p}\,}
\newcommand{\convas}{\,\mathop \rightarrow \limits^{a.s.}\,}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\pdf}{\emph{pdf}}
\newcommand{\mrv}{\emph{mrv}}
\newcommand{\rv}{\emph{rv}}


%%%%%%%%%%%%%%%%%%%%%%  Kernel related  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}
\newcommand{\HSIC}{\ensuremath{\mathrm{HSIC}}}
\newcommand{\HSICb}{\ensuremath{\widehat{\mathrm{HSIC}}_b}}
\newcommand{\HSICu}{\ensuremath{\widehat{\mathrm{HSIC}}_u}}
\newcommand{\MMD}{\ensuremath{\mathrm{MMD}}}
\newcommand{\convhil}[1]{\,\mathop \rightarrow \limits^{#1}\,}
\newcommand{\convuni}{\rightrightarrows}


%%%%%%%%%%%%%%%%%%%%%%  BOMC related  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\idf}{{\tt idf}}
\newcommand{\tp}{\ensuremath{\mathrm{tp}}}
\newcommand{\fn}{\ensuremath{\mathrm{fn}}}
\newcommand{\fp}{\ensuremath{\mathrm{fp}}}
\newcommand{\tpb}{\ensuremath{\overline{\text{tp}}}}
\newcommand{\fnb}{\ensuremath{\overline{\text{fn}}}}
\newcommand{\fpb}{\ensuremath{\overline{\text{fp}}}}
\newcommand{\pre}{\ensuremath{\mathrm{Pre}}}
\newcommand{\rec}{\ensuremath{\mathrm{Rec}}}
\newcommand{\fs}{\ensuremath{\mathrm{F-score}}}
\newcommand{\opt}{\ensuremath{\mathrm{opt}}}

\newcommand{\topics}{{\tt topics}}
\newcommand{\industries}{{\tt industries}}
\newcommand{\regions}{{\tt regions}}
\newcommand{\ip}{{\tt ip}}
\newcommand{\category}{{\tt category}}
\newcommand{\svmbb}{{\tt SVM\_Batch}}
\newcommand{\lasvm}{{\tt LaSVM}}
\newcommand{\larank}{{\tt LaRank}}
\newcommand{\svmstruct}{$\text{\tt SVM}^{\text{\tt Struct}}$}
\newcommand{\svmperf}{{\tt SVMPerf}}
\newcommand{\bomccmn}{{\tt BOMC\_CMN}}
\newcommand{\bomcsam}{{\tt BOMC\_Sample}}
\newcommand{\bomc}{{\tt BOMC}}
\newcommand{\pasagg}{{\tt PA}}
\newcommand{\paonline}{{\tt PA\_OnlineCV}}
\newcommand{\pabatch}{{\tt PA\_BatchCV}}
\newcommand{\bomcind}{{\tt BOMC\_IND}}
\newcommand{\bomcindcmn}{{\tt BOMC\_IND\_CMN}}
\newcommand{\bomcindsam}{{\tt BOMC\_IND\_Sample}}
\newcommand{\trueskill}{TrueSkill$^{\text{TM}}$}
\newcommand{\svmlight}{\ensuremath{\mathrm{SVM}^{\mathrm{light}}}}


%%%%%%%%%%%%%%%%%%%%%%  Nesterov related  %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\grad}{{\nabla}}
\newcommand{\gradbar}{{\bar{\nabla}}}
\newcommand{\mbarr}{{\overline{M(r)}}}
\newcommand{\card}{{\mathrm{card }}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\emp}{{\mathrm{emp}}}
\newcommand{\core}{{\mathrm{core}}}
\newcommand{\zerob}{{\mathbf{0}}}
\newcommand{\co}{{\mathrm{co}}}
\newcommand{\intr}{{\mathrm{int}}}
\newcommand{\bd}{{\mathrm{bd}}}
\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
\newcommand{\strcvx}{{\textit{s.c.}}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\cp}{\mathrm{cp}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\err}{{\sf err}}
\newcommand{\Xtr}{X_{\text{train}}}
\newcommand{\Xnew}{X_{\text{rep}}}
\newcommand{\Ctr}{{C_{\text{train}}}}
\newcommand{\yvectr}{{\yvec_{\text{train}}}}
\newcommand{\wcrf}{{\wvec_{\text{CRF}}}}
\newcommand{\wnode}{{\wvec_{\text{node}}}}
\newcommand{\wedges}{{\wvec_{\text{edge}}}}

